Information theoretic underpinning of self-supervised learning by clustering

Self-supervised learning (SSL) is recognized as an essential tool for building foundation models for Artificial Intelligence applications. The advances in SSL have been made thanks to vigorous arguments about the principles of SSL and through extensive empirical research. The aim of this paper is to contribute to the development of the underpinning theory of SSL, focusing on the deep clustering approach. By analogy to supervised learning, we formulate SSL as K-L divergence optimization. The mode collapse is prevented by imposing an optimisation constraint on the teacher distribution. This leads to normalization using inverse cluster priors. We show that using Jensen inequality this normalization simplifies to the popular batch centering procedure. Distillation and centering are common {heuristics-based} practices in SSL, {but our work underpins them theoretically.} The theoretical model developed not only supports specific existing successful SSL methods, but also suggests directions for future investigations.

==> sec/Algorithm1b.tex <==
\begin{algorithm}[ht] 
	\caption{ Algorithm 1}
	\label{algo1:llrr}
	\hspace*{0.2in} {\bf Input:} $X,   K, \tau_T, \tau_S, n_e, n_B, N$. 
	\begin{algorithmic}[1]
		\State {\bf Initialize:} $\tau_T, \tau_S, K, n_e, n_B$ \\ 
 % \hspace{0.5cm} $Q(i)=\frac{1}{K}$\\
        \text{random} $\theta_T,\theta_S, W_T, W_S,  $ 
		\For{ until convergence}
        \State $\theta=\alpha\theta_T + (1-\alpha)\theta_S$
        \State $W= \alpha W_T+(1-\alpha)W_S$
        \State $\theta_T=\theta$
        \State $W_T=W$
        \State update prior  \\ 
    \hspace{0.5cm} $Q(y)=\frac{1}{N}\sum_{j=1}^NP(y|\mathbf{z}_j)_{|\theta_T,W_T, \tau_T}, \forall y, j $
        \For{$l=1,...,n_e$}
        \For{$h=1,....,n_I$}
		\State \text{random}$X_B\epsilon X $
		\State $\max_{\theta_S,W_S} \sum_j \sum_y Q(y|\mathbf{z}_j)\log P(y|\mathbf{z}_j)_{|\theta_S,W_S, \tau_S} $ \\
  \hspace{1cm} where $Q(y|\mathbf{z}_j) =\frac{P(y|\mathbf{z}_j)_{|\theta_T, W_T, \tau_T}}{Q(y)} $ \\
  \hspace{1cm} $\mathbf{z}_j\epsilon X_B$
    \EndFor
    \EndFor
		\EndFor 
	\end{algorithmic}
\hspace{0.2in}  {\bf Output:} $\theta_S, W_S$
\end{algorithm}






==> sec/existing.tex <==
Sansone \cite{sansone2025} formulates SSL as optimisation of the log likelihood of the joint distribution of representations of the pairs of views of training  samples. He shows that this formulation can be related to  

==> sec/stability.tex <==
The key question is, why should this iterative process result in learning, and under what conditions? We know that the alternating direction optimisation method in each step will improve our objective function. However, to present a more convincing argument, let us look at the gradient in (\ref{it4}) in more detail. The product $Q(1-P)$ is a gradient weighting coefficient, which approaches zero when $Q$ and $P$ approach $1$ (or zero). This raises the question, whether the weight associated with the cluster with the highest probability will continue to dominate the gradient direction until convergence. To show that, let the teacher probability $Q_i=\max_y Q(y|\mathbf{z})$ at point $\mathbf{z}$ and $Q_k$ be the runner up. Let us assume that $Q_i\ge P_i$ by margin $\Delta_i$. This is reasonable, as $P_i$ will be catching up with $Q_i$. By the same assumption, $Q_k\leq P_k$ by margin $\Delta_k$. It is straightforward to show that the gradient weighting coefficient for cluster $i$ will always satisfy
\begin{equation}
\label{it8a}
(P_i + \Delta_i)(1-P_i) \ge (P_k-\Delta_k)(1-P_k)
\end{equation}
Expanding the products and rearranging we have 
\begin{equation}
\label{itA2}
(P_i-P_k)(1-P_i+P_k) +\Delta_i (1-P_i)+\Delta_k(1-P_k) \ge 0
\end{equation}
In (\ref{itA2}) all factors in the products are greater or equal to zero, hence the condition in (\ref{it8a}) is satisfied.
Now what will guarantee that the assumption $Q_i > P_i$ holds? Clearly, in the worst case scenario, at the point of teacher update, $Q_i = P_i$. However, referring to the numerator of (\ref{it8}) when updating (\ref{it7}), we can make teacher probability greater than student's either by setting a higher temperature for the teacher, i.e $\frac{1}{\tau_T}> \frac{1}{\tau_S}$, or by modifying the input sample by augmentation. Then the condition can be written as 
\begin{equation}
    \label{it9}
 \frac{1}{\tau_T}{(\mathbf{z}^T\mathbf{w}_i)} > \frac{1}{\tau_S}{(\tilde{\mathbf{z}}^T\mathbf{w}_i)}  
\end{equation}
where $\tilde{\mathbf{z}}$ is the more challenging view used by the student, corresponding to a small crop of the input image, or masked input. 

The above analysis and argument reflects the common practice in SSL: The weight vectors are normalised to a unit norm, the data distribution is scaled to a unit standard deviation, the temperature of the teacher is higher than that of a student and for every training instance $\mathbf{x}$ the student is fed its augmented version $\tilde{\mathbf{x}}$. 

We have derived the conditions under which the the learning process will iteratively improve the objective function. However, the learning could lead to a mode collapse. This tendency can be prevented by regularisation. This will be the topic of discussion in the next section. 


==> temperature.tex <==
\subsection{Temperature}
The information theoretic formulation of the self-supervised learning problem led to distillation, with clear roles defined for the student and teacher. The alternating direction optimisation approach also determined the nature of asymmetry between the two networks. So far we have refrained from discussing the choice of temperature to enable learning. The merits of temperature differential have already been discussed in the previous section.  %We do not subscribe to that school of thought, because the use of EM algorithm, for  a fixed set of network parameters, will automatically sharpen the teacher distribution by virtue of the iterative update of the cluster weight vectors. The EM algorithm has an additional advantage over the gradient method of optimising $Q(i|\mathbf{z})$, namely that its driving force does not diminish when $P(i|\mathbf{z},w_i)$ approaches unity. EM will converge to a stable solution for $w_i, \forall i$ after a few iterations. \textcolor{red}{Is this a good idea? What is the implication on the fixed weight vector approach?} The choice of temperature will actually impact on the behaviour of the EM algorithm. For $\tau$ approaching zero, EM will operate as the k-means algorithm. 

%The learning behaviour of the self-supervised system will be investigated by ablation studies.
%In any case, it cannot be overemphasised that we would not exclude a temperature differential, if its pragmatic use led to a better performance. Accordingly, the supervisory signal update would be defined 
%One such inducement is to sharpen $Q(y|\mathbf{z})$ at each update. This can easily be done by using a higher temperature $\tau^*$ for the supervisory signal distribution update, i.e.
%\begin{equation}
%    \label{it8}
%    P^*(y|\mathbf{z},w_y) =\frac{\exp{\%{\mathbf{z}^Tw_y/\tau^*}\}}{\sum_i^m %\exp{\{\mathbf{z}^Tw_i/\tau^*}\}}
%\end{equation}
%\begin{equation}
 %   \label{it8}
  %  Q(y|\mathbf{z}) %\propto\frac{P(y|\mathbf{z},W)_{|\theta_%T, W_T, \tau_T}}{Q(y)}
%\end{equation}
%where $\tau_T$ indicates that the softmax posterior in $Q(y|\mathbf{z})$ is computed at the teacher temperature, that differs from that of the student. This immediately raises the question, namely whether the cluster prior probabilities needed for normalisation should also be computed at the teacher temperature. This makes the theoretical development rather messy, and without any principled justification, we opt for the simple option of keeping the temperature the same for the two networks. The merit of any differential will be investigated by ablation studies in Section \ref{ablation}.

As high temperature sharpens softmax, an undue level would make it impossible to define the notion of similarity. In deep learning, by changing the network parameters, we can drive all training samples either close or far away from each other arbitrarily. To define a notion of similarity, we want to choose temperature $\tau$ so that similar samples are assigned congruent probabilities of belonging to the same cluster by the predictor. %In image and video analysis, such samples are created by taking multiple views $\mathbf{x}_i, \ i=1,n_v$ for each sample $\mathbf{x}$ and forcing all the corresponding embeddings $\mathbf{z}_i, \ i=1,...,n_v$ to the same cluster by means of sharing the same supervisory signal $Q(y|\mathbf{z})$. These views can be global, or local. However, such a strategy would not address the problem that multiple instances in the training set, belonging to the same class, should be assigned to the same cluster. It is therefore more appropriate to define the notion of a sample affinity objectively, in an absolute sense. 
%For global views, 
This can be done in terms of the cosine similarity in the argument of the softmax function. It is reasonable to assume that sample embeddings within a certain angular interval with respect to their closest cluster means, e.g. $66^o$,  would be considered as similar. This would define the cosine similarity between the embeddings and the corresponding weight vectors of their closest shared cluster to be  greater than $0.4$. For the worst case scenario of the samples on the boundary between two competing clusters with cosine similarity of $0.4$ the cluster assignment probability should be of the order of $0.5$. Noting that these samples should also score low with respect to the other clusters, that is we expect them to be orthogonal to the weight vectors of these clusters, with the exception of the closest competing cluster, we get for softmax the condition that
\begin{equation}
    \label{it22}
    P(y|\mathbf{z})=\frac{\exp^{0.4\tau^{-1}}}{\exp^{0.4\tau^{-1}}+K-1}=0.5
\end{equation}
This suggests that for a small number of clusters, say $K=10$, the temperature should be set around $\tau=0.2$. In self supervised learning the number of clusters needed to represent all the training data would be much higher. In Dino \cite{caron2018deep}, for instance, the number of clusters is set to $64,000$. However, experimental studies reported in the literature suggest that, as selfsupervised learning is striving to find a balance between the notion of similarity and uniform cluster occupancy, not all the clusters are necessarily populated, and effective solutions in terms of a much smaller number of clusters can be found. For a coarser representation in terms of, say, just $K=4000$ clusters, the temperature for the supervision signal estimation (teacher network) should be set around $\tau=0.05$. Referring to our discussion regarding the relationship of teach and student temperatures, the prediction probability should be computed at a lower temperature than $0.05$, say, around $0.1$. These ballpark figures will be validated in the supplementary material. In any case they are pretty consistent with the empirically based practice. It is useful to note where they come from.




%At this point, a comment is in order. One of the heuristic approaches used for self supervised learning is distillation, where a teacher network defines the learning goals for a student network. Referring to the K-L divergence, this is equivalent to considering the supervisory signal as the teacher network output. Typically, the teacher network is updated by passing on the parameters of the student network to the teacher.  


